Energy-Aware Dynamic Neural Inference

The growing demand for intelligent applications beyond the network edge, coupled with the need for sustainable operation, are driving the seamless integration of deep learning (DL) algorithms into energy-limited, and even energy-harvesting end-devices. However, the stochastic nature of ambient energy sources often results in insufficient harvesting rates, failing to meet the energy requirements for inference and causing significant performance degradation in energy-agnostic systems. To address this problem, we consider an on-device adaptive inference system equipped with an energy-harvester and finite-capacity energy storage. We then allow the device to reduce the run-time execution cost on-demand, by either switching between differently-sized neural networks, referred to as multi-model selection (MMS), or by enabling earlier predictions at intermediate layers, called early exiting (EE). The model to be employed, or the exit point is then dynamically chosen based on the energy storage and harvesting process states. We also study the efficacy of integrating the prediction confidence into the decision-making process. We derive a principled policy with theoretical guarantees for confidence-aware and -agnostic controllers. Moreover, in multi-exit networks, we study the advantages of taking decisions incrementally, exit-by-exit, by designing a lightweight reinforcement learning-based controller. Experimental results show that, as the rate of the ambient energy increases, energy- and confidence-aware control schemes show approximately 5% improvement in accuracy compared to their energy-aware confidence-agnostic counterparts. Incremental approaches achieve even higher accuracy, particularly when the energy storage capacity is limited relative to the energy consumption of the inference model.

==> figures/introduction/computing_paradigms/early_exiting_incremental.tex <==
\newcommand{\tx}{-1.7}
\newcommand{\ty}{1.7}
\newcommand{\sx}{0.}
\newcommand{\sy}{1.5}
\newcommand{\imgy}{2.95}

\usetikzlibrary{circuits.ee.IEC}

\begin{tikzpicture}[
    circuit ee IEC,
    set make contact graphic= var make contact IEC graphic
    ]
    % Control rectangle
    \draw[draw=black, dashed, fill=Apricot!20] (-0.75,0.58) rectangle ++(2.3,.36);
    \node[black] at (0.4,.58+.36/2) {\small Control};
    \draw[-{Latex[open, length=5pt]}, BlueViolet, thick] (0.45, .58) -- (.45, 0.3);
    % \draw[-{Diamond[open, length=6pt]}, purple!50!black, thick] (0.05, .58) -- (0.05, 0.3);
    % \draw[-{Diamond[open, length=6pt]}, purple!50!black, thick] (0.8, .58) -- (.8, 0.3);
    
    
    % DNNEE rectangle
    \draw[draw=black, fill=red!30] (-0.6,-0.6) rectangle ++(2.,.9);
 
    % Ys
    \node[black!50] at (0.,-1.3) {\small$\hat{\ry}^{(1)}$};
    \node[black] at (1.,-1.3) {\small$\hat{\ry}^{(2)}$};
    \node[black!50] at (2.,-1.3) {\small$\hat{\ry}^{(3)}$};

    % Body
    \draw[black] (-1.5, -0.135) -- (-.35,-0.135);
    % \draw[black] (-1.5, -0.1) node[fill, circle, inner sep=1pt]{} -- (-.35,-0.1);
    \draw[black] (.15, -0.135) node[fill, circle, inner sep=1pt]{} -- (.65,-0.135);
    \draw[black] (1.15, -0.135) node[fill, circle, inner sep=1pt]{} -- (2,-0.135);

    % Connecting arrows to Ys
    \draw[black, ->] (.65+0.353-1, -0.503) node[fill, circle, inner sep=1pt]{} -- (.65+0.353-1,-1);
    \draw[black, ->] (.65+0.353, -0.503) node[fill, circle, inner sep=1pt]{} -- (.65+0.353,-1);
    \draw[black, ->] (.65+0.353+1, -0.135) -- (.65+0.353+1,-1);

   % White nodes and bending arrows
    \draw (-0.35, -0.135) node[fill=white, draw, circle, inner sep=1pt]{} -- ++ (0.5, 0);
    \draw[-{Latex[open, length=5pt]}, BlueViolet, thick] (-0.18, 0+0.1) to[bend left] (-.19, -0.4);
    
    % White nodes and bending arrows
    \draw (0.65, -0.135) node[fill=white, draw, circle, inner sep=1pt]{} -- ++ (0.353, -0.353);
    \draw[-{Latex[open, length=5pt]}, BlueViolet, thick] (.8, 0+0.1) to[bend left] (.75, -0.4);

    % Picture -0.1
    \node[inner sep=0] at (-1.8,-0.135) {\includegraphics[scale=0.12]{figures/mnist5.png}};
    \node[black] at (-1.05,-0.3) {\small$\rw$};

    % Battery Block
    \draw[draw=black ] (-1.05,1.1) rectangle node[]{\small ES $\rb$} ++(1.2,0.4);
    \draw[->] (-1.05+1.2, 1.3) -- +(.25,0) -- (-.8+1.2, 0.94);

    % Harvesting Block
    \draw[draw=black ] (.8,1.1) rectangle node[]{\small EH $\rh$} ++(1.2,0.4);
    \draw[->] (.8, 1.3) -- +(-.25,0) -- (.8-0.25, 0.94);
    % \draw[->] (\basex+1.8,\basey-\modeloffset-1+0.2) -- +(-.25,0) -- (\basex+1.8-0.25,\basey-\modeloffset-0.3);

\end{tikzpicture}


==> figures/introduction/computing_paradigms/early_exiting_oneshot.tex <==
\newcommand{\tx}{-1.7}
\newcommand{\ty}{1.7}
\newcommand{\sx}{0.}
\newcommand{\sy}{1.5}
\newcommand{\imgy}{2.95}

\usetikzlibrary{circuits.ee.IEC}
\usetikzlibrary {arrows.meta}

\begin{tikzpicture}[
    circuit ee IEC,
    set make contact graphic= var make contact IEC graphic
    ]
    % Control rectangle
    \draw[draw=black, dashed, fill=Apricot!20] (-0.75,0.58) rectangle ++(2.3,.36);
    \node[black] at (0.4,.58+.36/2) {\small Control};
    % \draw[-{Diamond[open, length=6pt]}, purple!50!black, thick] (0.05, .58) -- (0.05, 0.3);
    \draw[-{Latex[open, length=5pt]}, BlueViolet, thick] (0.45, .58) -- (.45, 0.3);
    
    % DNNEE rectangle
    \draw[draw=black, fill=red!30] (-0.6,-0.6) rectangle ++(2.,.9);
 
    % Ys
    \node[black!50] at (0.,-1.3) {\small$\hat{\ry}^{(1)}$};
    \node[black] at (1.,-1.3) {\small$\hat{\ry}^{(2)}$};
    \node[black!50] at (2.,-1.3) {\small$\hat{\ry}^{(3)}$};

    % Body
    \draw[black] (-1.5, -0.135) -- (-.35,-0.135);
    \draw[black] (.15, -0.135) node[fill, circle, inner sep=1pt]{} -- (.65+0.353-0.4, -0.135) -- (.65+0.353, -0.503);
    \draw[black] (.65+0.353-1, -0.1+0.303) node[fill, circle, inner sep=1pt]{} -- (1.6, -0.1+0.303) -- (2,-0.2);

    % Connecting arrows to Ys
    \draw[black, ->] (.65+0.353-1, -0.503) node[fill, circle, inner sep=1pt]{} -- (.65+0.353-1,-1);
    \draw[black, ->] (.65+0.353, -0.503) -- (.65+0.353,-1);
    \draw[black, ->] (.65+0.353+1, -0.2) -- (.65+0.353+1,-1);

   % White nodes and bending arrows
    \draw (-0.35, -0.135) node[fill=white, draw, circle, inner sep=1pt]{} -- ++ (0.5, 0);
    \draw[-{Latex[open, length=5pt]}, thick, BlueViolet] (-0.18, 0+0.1) to[bend left] (-.19, -0.4);

    % Picture -0.1
    \node[inner sep=0] at (-1.8,-0.135) {\includegraphics[scale=0.12]{figures/mnist5.png}};
    \node[black] at (-1.05,-0.3) {\small$\rw$};

    % Battery Block
    \draw[draw=black ] (-1.05,1.1) rectangle node[]{\small ES $\rb$} ++(1.2,0.4);
    \draw[->] (-1.05+1.2, 1.3) -- +(.25,0) -- (-.8+1.2, 0.94);

    % Harvesting Block
    \draw[draw=black ] (.8,1.1) rectangle node[]{\small EH $\rh$} ++(1.2,0.4);
    \draw[->] (.8, 1.3) -- +(-.25,0) -- (.8-0.25, 0.94);
    % \draw[->] (\basex+1.8,\basey-\modeloffset-1+0.2) -- +(-.25,0) -- (\basex+1.8-0.25,\basey-\modeloffset-0.3);

\end{tikzpicture}


==> figures/introduction/computing_paradigms/multi_model_selection.tex <==
% \newcommand{\tx}{-1.7}
% \newcommand{\ty}{1.7}
% \newcommand{\sx}{0.}
% \newcommand{\sy}{1.2}
% \newcommand{\imgy}{3.2}
% \newcommand{\upoffset}{0.1}


% \begin{tikzpicture}[scale=1.]
%     \draw[draw=black, fill=red!30] (\sx-0.2,\sy+1.2-\upoffset) rectangle ++(.4,0.3);
%     \draw[draw=black, fill=red!30] (\sx+1-0.2,\sy+1.2-\upoffset) rectangle ++(.4,0.3);
%     \draw[draw=black, fill=red!30] (\sx+2-0.2,\sy+1.2-\upoffset) rectangle ++(.4,0.3);

%     \fill[fill=blue!20, fill opacity=0.2] (\sx-1.7,\sy+0.2) rectangle (\sx+2.5,\sy-1.2);
%     % \fill[fill=blue!20, fill opacity=0.4] (-1.7,1.) rectangle (2.5,.3);
    
%     \node[black] at (\sx+0.,\sy+.7-\upoffset) {\small$\text{Acc}_{1}$};
%     \node[black] at (\sx+1.,\sy+.7-\upoffset) {\small$\text{Acc}_{2}$};
%     \node[black] at (\sx+2.,\sy+.7-\upoffset) {\small$\text{Acc}_{3}$};
%     % \node[black] at (3.,2.2) {$\hat{Y}_t^{(3)}$};
    
%     \node[black] at (-1.5,2.2) {$X_t$};

%     % Exits' arrows 
%     \draw[black, ->] (\sx+0, \sy+1.2-\upoffset) -- (\sx+0,\sy+.9-\upoffset);
%     \draw[black, ->] (\sx+1, \sy+1.2-\upoffset) -- (\sx+1,\sy+.9-\upoffset);
%     \draw[black, ->] (\sx+2, \sy+1.2-\upoffset) -- (\sx+2,\sy+.9-\upoffset);
%     % \draw[black, ->] (3, 2.95) -- (3,2.5);
%     %\draw[black] (\sx+1.5, 2.95) -- (\sx+2,2.95);
%     \draw[black, ] (\sx-1.5, \imgy) -- (\sx+1,\imgy);

%     \node[ state, fill=gray!5, inner sep=1pt,minimum size=0pt] at (\sx,\sy) (A1) {\small$s_t$};
%     \node[ state, fill=gray!5, inner sep=1pt,minimum size=0pt] at (\sx,\sy-1.5) (C1) {\tiny$s_{t+1}$};
%     \node[ state, fill=gray!5, inner sep=1pt,minimum size=0pt] at (\sx+1,\sy-1.5) (C2) {\tiny$s_{t+1}$};
%     \node[ state, fill=gray!5, inner sep=1pt,minimum size=0pt] at (\sx+2,\sy-1.5) (C3) {\tiny$s_{t+1}$};

%     \path
%     % Idle
%     (A1) edge[below, ->, blue, ]		        node{}	(C1)
%     (A1) edge[below,->, purple, bend left ]		            node{}	(C2)
%     (A1) edge[below,->, orange, bend left ]		            node{}	(C3);

%     \node[inner sep=0] at (-1.5,\imgy) {\includegraphics[scale=0.12]{figures/mnist5.png}};

%     \draw[draw=black, <->] (\sx-1.7,\sy+0.2) -- (\sx-1.7,\sy+0.2-1.4);
%     \node[black] at (-1.88,1.) {\footnotesize$t$};
    
%     % \draw[draw=black, dashed] (-1.5,1.) -- (2.5,1.);
%     % \draw[draw=black, dashed] (-1.5,.3) -- (2.5,.3);

%     % Legend
%     \fill[fill=blue, fill opacity=1] (\sx+1.6,\sy+0.1) rectangle (\sx+1.75,\sy+0.07);
%     \node[black] at (\sx+2.1,\sy+.085) {\tiny$A_{t}$= $1$};
%     \fill[fill=purple, fill opacity=1] (\sx+1.6,\sy-0.1) rectangle (\sx+1.75,\sy-0.13);
%     \node[black] at (\sx+2.1,\sy-0.115) {\tiny$A_{t}$= $2$};
%     \fill[fill=orange, fill opacity=1] (\sx+1.6,\sy-.3) rectangle (\sx+1.75,\sy-0.33);
%     \node[black] at (\sx+2.1,\sy-0.315) {\tiny$A_{t}$= $3$};

% \end{tikzpicture}

\newcommand{\sizemodelbox}{0.45}
\newcommand{\sizemodelboxy}{0.35}
\newcommand{\modeloffset}{0.5}
\newcommand{\basex}{-0.2}
\newcommand{\basey}{0}


\usetikzlibrary{circuits.ee.IEC}

\begin{tikzpicture}[
    circuit ee IEC,
    set make contact graphic= var make contact IEC graphic
    ]

    %% Controller box
    \draw[draw=black,dashed, fill=Apricot!20] (\basex+.8,\basey-\modeloffset-0.2) rectangle ++(1.2,1.6);
    \node[black] at (\basex+0.8+1.2/2,\basey+\modeloffset+0.25) {\small Control};

    % Battery Block
    \draw[draw=black] (\basex-0.2,\basey+\modeloffset+0.6) rectangle node[]{\small ES $\rb$} ++(1.2,0.4);
    \draw[->] (\basex+1.,\basey+\modeloffset+0.6+0.2) -- +(.25,0) -- (\basex+1.+0.25,\basey+\modeloffset+0.4);

    % Harvesting Block
    \draw[draw=black] (\basex+1.8,\basey+\modeloffset+0.6) rectangle node[]{\small EH $\rh$} ++(1.2,0.4);
    \draw[->] (\basex+1.8,\basey+\modeloffset+0.6+0.2) -- +(-.25,0) -- (\basex+1.8-0.25,\basey+\modeloffset+0.4);
    
    % Picture
    \node[inner sep=0, anchor=east] at (0.05,0) {\includegraphics[scale=0.12]{figures/mnist5.png}};
    \node[black] at (0.3,-.2) {\small$\rw$};

    % Models
    \draw[draw=black, fill=red!30] (2,\modeloffset-\sizemodelboxy/2) rectangle node[]{\footnotesize$f_1$} ++(\sizemodelbox,\sizemodelboxy);
    \draw[draw=black, fill=red!30] (2,\modeloffset-0.5-\sizemodelboxy/2) rectangle node[]{\footnotesize$f_2$} ++(\sizemodelbox+0.2,\sizemodelboxy);
    \draw[draw=black, fill=red!30] (2,\modeloffset-1-\sizemodelboxy/2) rectangle node[]{\footnotesize$f_3$} ++(\sizemodelbox+0.4,\sizemodelboxy);
    
    % Input
    \draw (-0.1, \basey) -- (\basex+1, \basey) node[circle, fill, inner sep=1pt] {};
    
    % switch
    \draw (\basex+1, \basey) -- ++ (\modeloffset, \modeloffset);
    \draw[-{Latex[open, length=5pt]}, BlueViolet, thick] (\basex+1.2, \basey+0.4) to[bend left] (\basex+1.3, \basey-0.36);

    % 
    \draw (\basex+1.5, \basey+\modeloffset) node[circle, fill=white, draw, inner sep=1pt]{} -- (2., \basey+\modeloffset);
    \draw (\basex+1.707, \basey) node[circle, fill=white, draw, inner sep=1pt]{} -- (2, \basey);
    \draw (\basex+1.5, \basey-\modeloffset) node[circle, fill=white, draw, inner sep=1pt]{} -- (2., \basey-\modeloffset);


    \draw[->] (2+\sizemodelbox, \basey+\modeloffset) -- ++ (.1+0.6, 0);
    \draw[->] (2+\sizemodelbox+0.2, \basey) -- ++ (.1+0.4, 0);
    \draw[->] (2+\sizemodelbox+0.4, \basey-\modeloffset) -- ++ (.1+0.2, 0);

    \node[black] at (3.1+0.4,.5) {\small$\hat{\ry}^{(1)}$};
    \node[black!50] at (3.1+0.4,0) {\small$\hat{\ry}^{(2)}$};
    \node[black!50] at (3.1+0.4,-.5) {\small$\hat{\ry}^{(3)}$};
\end{tikzpicture}


==> figures/introduction/local_vs_offload.tex <==
\usepgfplotslibrary{fillbetween}
\begin{tikzpicture}

\begin{axis}[
    width=7cm,
    height=6cm,
    ymin=-10,
    ymax=23.63,
    xmin=0,
    xmax=71, 
    xlabel={Bitrate [MB/s]},
    ylabel={Tx Power [dBm]},
    ticks=none,
    axis x line=bottom,axis y line=left,
    axis line style = thick,
    axis on top,
]
\addplot [
    %draw=none,
    domain=0.00001:71,
    samples=200, 
    color=NavyBlue,
    name path=curve,
    dashed,
    thick
]
{10*log10(0.56*x*1e6/1990656)};
%\addlegendentry{\(x^2 - 2x - 1\)}

\addplot[thick, samples=2, NavyBlue, dashed, name path=vertical] coordinates {(35.54742857142857,-20)(35.54742857142857,25)};

\node at (axis cs:16,15) [anchor=south, align=center, font=\bfseries\footnotesize\selectfont] {Local\\Computing};
\node at (axis cs:16,10.5) [anchor=south, align=center, font=\tiny\selectfont] {$E_{\text{local}}\leq E_{\text{offload}}$\\$T_{\text{local}}\leq T_{\text{offload}}$};

\node at (axis cs:53,14) [anchor=south, align=center, font=\tiny\selectfont] {$E_{\text{local}}\leq E_{\text{offload}}$\\$T_{\text{local}}\geq T_{\text{offload}}$};

\node at (axis cs:53,-3+2) [anchor=south, align=center, font=\bfseries\footnotesize\selectfont] {Data\\Offloading (MEC)};
\node at (axis cs:53,-7+2) [anchor=south, align=center, font=\tiny\selectfont] {$E_{\text{local}}\geq E_{\text{offload}}$\\$T_{\text{local}}\geq T_{\text{offload}}$};

%\node at (axis cs:19,-3) [anchor=south, align=center, font=\bfseries\footnotesize\selectfont] {Data\\Offloading};
\node at (axis cs:16,-5) [anchor=south, align=center, font=\tiny\selectfont] {$E_{\text{local}}\geq E_{\text{offload}}$\\$T_{\text{local}}\leq T_{\text{offload}}$};

\addplot[samples=2, blue, name path=hub] coordinates {(-10,40)(100,40)};
\addplot[samples=2, blue, name path=hlb] coordinates {(-10,-40)(100,-40)};


\addplot[green!20] fill between[ 
    of = curve and hub,
    soft clip={domain=0:35.54742857142857},
];

\addplot[MidnightBlue!30] fill between[ 
    of = curve and hlb,
    soft clip={domain=35.54742857142857:100},
];
% \addplot fill between[ 
%     of = vertical and curve,
%     split, % calculate segments
%     every even segment/.style = {green!20},
%     every odd segment/.style = {white},
% ];
\end{axis}
\end{tikzpicture}

==> figures/results/performance/accuracy_capacity.tex <==
% \usetikzlibrary{
%         pgfplots.colorbrewer,
%     }
% \usepgfplotslibrary{colormaps}
\usetikzlibrary{fit,shapes}

\begin{tikzpicture}[every mark/.append style={mark size=1.5pt},]
\begin{axis}[
    xlabel={\gls{es} Maximum Capacity, $b_{\text{max}}$},
    ylabel={Average Accuracy, $\rho$},
    % no markers,
    every axis plot/.append style={thick},
    legend columns=2,
    legend style={
            font=\scriptsize,
            at={(0.95,0.06)},
            anchor=south east,
        },
    legend cell align={left},
    symbolic x coords={3,5,10,20,30},
    grid style={line width=.1pt, draw=gray!10},
    major grid style={dashed, line width=.2pt,draw=gray!50},
    ymajorgrids=true,
    % width=7cm,
    % height=7.2cm
    % xmajorgrids=true,
]   
    \addplot[color=Purple, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data1.csv};
    % \addlegendentry{One-shot EE (DQN)}

    \addplot[color=Blue, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data2.csv};
    % \addlegendentry{One-shot EE (Oracle)}

    \addplot[color=Melon, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data3.csv};
    % \addlegendentry{Incremental Sample-Agnostic EE}

    \addplot[color=LimeGreen, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data4.csv};
    % \addlegendentry{One-shot Random}

    \addplot[color=RedOrange, mark=triangle*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data5.csv};
    % \addlegendentry{Incremental Sample-Aware EE}

    \addplot[color=Green, mark=triangle*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data6.csv};
    % \addlegendentry{Incremental Random}

    \addplot[color=Aquamarine, mark=triangle*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_capacity/data7.csv};
    % \addlegendentry{Incremental Sample-Aware EE (DQN)}

    
    % Confidence Intervals
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci1.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci1.csv};
    \addplot [opacity=0.1, color=Purple] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci2.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci2.csv};
    \addplot [opacity=0.1, color=Blue] fill between[of=lower and upper];

    
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci3.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci3.csv};
    \addplot [opacity=0.1, color=Melon] fill between[of=lower and upper];

    
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci4.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci4.csv};
    \addplot [opacity=0.1, color=LimeGreen] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci5.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci5.csv};
    \addplot [opacity=0.1, color=RedOrange] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci6.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci6.csv};
    \addplot [opacity=0.1, color=Green] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_capacity/ci7.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_capacity/ci7.csv};
    \addplot [opacity=0.1, color=Aquamarine] fill between[of=lower and upper];
    
    \node at (30,0.43) {\footnotesize Random};
    \draw[] (30,0.485) ellipse (0.2cm and .6cm);

    \node at (30,0.575) {\footnotesize \gls{iag}};
    \draw[] (30,0.61) ellipse (0.2cm and .3cm);
    
    \node at (30,0.725) {\footnotesize \gls{iaw}};
    \draw[](30,0.685) ellipse (0.2cm and .4cm);
    
    
\end{axis}


\end{tikzpicture}



==> figures/results/performance/accuracy_energy.tex <==
% \usetikzlibrary{
%         pgfplots.colorbrewer,
%     }
% \usepgfplotslibrary{colormaps}

\begin{tikzpicture}[every mark/.append style={mark size=.5pt},]
\begin{axis}[
    xlabel={Incoming Energy Rate, $\mu$},
    ylabel={Average Accuracy, $\rho$},
    no markers,
    every axis plot/.append style={thick},
    legend columns=2,
    legend style={
            font=\scriptsize,
            at={(.95,0.06)},
            anchor=south east,
        },
    legend cell align={left},
    % legend columns=1,
    xmin=0.25,
    xmax= 3.15,
    ymin=0.1,
    ymax=0.92,
    % width=7cm,
    % height=7.2cm
]   
    
    \addplot[color=Purple, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data1.csv};
    \addlegendentry{\gls{os}\gls{iaw}\gls{ee}-\gls{dqn}}

    \addplot[color=Blue, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data2.csv};
    \addlegendentry{\gls{os}\gls{iaw}\gls{ee}-oracle}

    \addplot[color=Melon, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data3.csv};
    \addlegendentry{\gls{mms}}

    \addplot[color=LimeGreen, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data4.csv};
    \addlegendentry{\gls{os}Rand}

    \addplot[color=RedOrange, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data5.csv};
    \addlegendentry{\gls{os}\gls{iag}\gls{ee}}

    \addplot[color=Green, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data6.csv};
    \addlegendentry{\gls{inc}Rand}

    \addplot[color=Aquamarine, mark=*] table [x=x, y=y, col sep=comma] {figures/results/performance/data_acc_energy/data7.csv};
    \addlegendentry{\gls{inc}\gls{iaw}\gls{ee}-\gls{dqn}}

    
    % Confidence Intervals
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci1.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci1.csv};
    \addplot [opacity=0.2, color=Purple] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci2.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci2.csv};
    \addplot [opacity=0.2, color=Blue] fill between[of=lower and upper];

    
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci3.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci3.csv};
    \addplot [opacity=0.2, color=Melon] fill between[of=lower and upper];

    
    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci4.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci4.csv};
    \addplot [opacity=0.2, color=LimeGreen] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci5.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci5.csv};
    \addplot [opacity=0.2, color=RedOrange] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci6.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci6.csv};
    \addplot [opacity=0.2, color=Green] fill between[of=lower and upper];


    \addplot [name path=upper, fill=none, draw=none] table [
    x=x, y=upper, col sep=comma]{figures/results/performance/data_acc_energy/ci7.csv};
    \addplot [name path=lower, fill=none, draw=none] table [
    x=x, y=lower, col sep=comma]{figures/results/performance/data_acc_energy/ci7.csv};
    \addplot [opacity=0.2, color=Aquamarine] fill between[of=lower and upper];

    \addplot[color=gray!40, dashed] plot coordinates {(0,.53)(1.,.53)};
    \addplot[color=gray!40, dashed] plot coordinates {(1,0)(1.,.53)};
    \node[] at (axis cs: 0.6,.56) {\small$\rho$@Exit1};

    
    \addplot[color=gray!40, dashed] plot coordinates {(0,.69)(2.,.69)};
    \addplot[color=gray!40, dashed] plot coordinates {(2,0)(2.,.69)};
    \node[] at (axis cs: 0.6,.72) {\small$\rho$@Exit2};


    \addplot[color=gray!40, dashed] plot coordinates {(3,0)(3.,.83)};
    \addplot[color=gray!40, dashed] plot coordinates {(0,.83)(3.,.83)};
    \node[] at (axis cs: .6,.86) {\small$\rho$@Exit3};
    
\end{axis}


\end{tikzpicture}


% \begin{tikzpicture}
% \begin{axis}[
%     xlabel={Incoming Energy Rate, $\mu$},
%     no markers,
%     colormap/hsv,
%     % every fill between plot/.style={
%     %     /pgfplots/area legend, /tikz/fill, cycle list/Dark2-7},
%     every axis plot/.append style={thick},
%     %cycle list/Dark2-7,
%     legend columns=2,
%     legend style={
%             font=\scriptsize,
%             at={(0.95,0.06)},
%             anchor=south east,
%             % draw=none,
%         },
% ]
%     \foreach \i/\C in {1/Purple, 2/Blue, 3/Melon, 4/LimeGreen, 5/RedOrange, 6/Green, 7/Aquamarine} {%
%         \edef\temp{%
%             \noexpand\addplot[color=\C] table [x=x, y=y, col sep=comma] {figures/results/performance/data/data\i.csv};
%             \noexpand\addlegendentry{Controller}}\temp%
%             \edef\temp{%
%             % Confidence Intervals
%             \noexpand\addplot [name path=upper, fill=none, draw=none] table [
%             x=x, y=upper, col sep=comma]{figures/results/performance/data/ci\i.csv};}\temp%

%             \edef\temp{%
%             \noexpand\addplot [name path=lower, fill=none, draw=none] table [
%             x=x, y=lower, col sep=comma]{figures/results/performance/data/ci\i.csv};}\temp%

%             \edef\temp{%
%             \noexpand\addplot [opacity=0.2, color=\C] fill between[of=lower and upper];}\temp%
%     }
% \end{axis}
% \end{tikzpicture}


